Energy Resolved Neutron Imaging for Strain Reconstruction using the Finite Element Method

A pulsed neutron imaging technique is used to reconstruct the residual strain within a polycrystalline material from Bragg edge strain images. This technique offers the possibility of a nondestructive analysis of strain fields with a high spatial resolution. A finite element approach is used to reconstruct the strain using the least square method constrained by the conditions of equilibrium. The procedure is developed and verified by validating for a cantilevered beam problem. It is subsequently demonstrated by reconstructing the strain from experimental data for a ring-and-plug sample, measured at the spallation neutron source RADEN at J-PARC in Japan. The reconstruction is validated by comparison with conventional constant wavelength strain measurements on the KOWARI diffractometer at ANSTO in Australia. It is also shown that the addition of a simple Tikhonov regularization can improve the reconstruction.

==> bib.bbl.tex <==
% Encoding: UTF-8
@article{review,
  author={R. Woracek and Javier Santisteban and Anna Fedrigo and Markus Strobl},
  title={Diffraction in neutron imaging —- A review},
  year={2018},
  journal={Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
  volume={878},
  pages={141--158},
  publisher={}}

@article{golub1999tikhonov,
  title={Tikhonov regularization and total least squares},
  author={Golub, Gene H and Hansen, Per Christian and O'Leary, Dianne P},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={21},
  number={1},
  pages={185--194},
  year={1999},
  publisher={SIAM}
}
@article{inverse_prob,
  author    = {W. R. B. Lionheart and P. J. Withers},
  title     = {Diffraction tomography of strain},
  booktitle = {Inverse Problems},
  year      = {2015},
  volume    = {31},
  pages     = {045005},
}

@article{Kirkwood2015,
author ={Henry J. Kirkwood and Shu Yan Zhang and Anton S. Tremsin and Alexander M. Korsunsky and Nikolaos Baimpas and Brian Abbey},
title={Neutron Strain Tomography using the Radon Transform},
journal={Materials Today: Proceedings},
year={2015},
volume  = {2},
pages   = {S414--S423},
issn    = {},
}


@inproceedings{Gregg2017TomographicRO,
	title={Tomographic reconstruction of residual strain in axisymmetric systems from Bragg-edge neutron imaging},
	author={Alexander Gregg and Johannes N. Hendriks and Christopher Wensrich and Michael H. Meylan},
	year={2017}
}


@article{Abbey,
  author  = {B. Abbey and Shu Yan Zhang and Wim.J.J. Vorster and Alexander M. Korsunsky},
  title   = {Feasibility study of neutron strain tomography},
  journal = {Procedia Engineering},
  year    = {2009},
  volume  = {1},
  pages   = {185--188},
  issn    = {},
}
@article{Abbey12,
	author  = {B. Abbey and Shu Yan Zhang and Wim.J.J. Vorster and Alexander M. Korsunsky},
	title   = {Reconstruction of axisymmetric strain distributions via neutron strain tomography},
	journal = {Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
	year    = {2012},
	volume  = {270},
	pages   = {28--35},
	issn    = {},
}
@inproceedings{Sharafutdinov1994INTEGRALGO,
	title={INTEGRAL GEOMETRY OF TENSOR FIELDS},
	author={Vladimir A. Sharafutdinov},
	year={1994}
}



@article{Bragg_edge,
  author  = {Hendriks, J. N. and Gregg, A. W. T. and Wensrich, C. M. and Tremsin, A. S. and Shinohara, T. and Meylan, M. and Kisi, E. H. and Luzin, V. and Kirsten, O.},
  title   = {Bragg-edge elastic strain tomography for in situ systems from energy-resolved neutron transmission imaging},
  journal = {Phys. Rev. Materials},
  year    = {2017},
  volume  = {1},
  pages   = {053802},
  issn    = {},
}


@book{Gaussian,
  author  = {C. E. Rasmussen and C. K. I. Williams},
  title   = {Gaussian Processes for Machine Learning},
  journal = {MIT Press},
  year    = {2006},
  pages   = {},
  issn    = {},
  }

@article{Gauss_prob,
  author  = {C. Jidling and Johannes Hendriks and Niklas Wahlström and Alexander Gregg and Thomas B. Schön and Christopher Wensrich and Adrian Wills},
  title   = {Probabilistic modelling and reconstruction of strain},
  journal = {Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
  year    = {2018},
  pages   = {141--155},
  issn    = {},
  }


@article{AIP,
  author    = {C. M. Wensrich and Kisi, Erich and Luzin, Vladimir and Kirstein, Oliver},
  title     = {Non-contact Measurement of the Stress within Granular Materials via Neutron Diffraction},
  journal = {AIP Conference Proceedings},
  year      = {2013},
  volume    = {1542},
  pages     = {441--444},
}
@article{granular,
	author    = {C. M. Wensrich and Kisi, Erich and Luzin, Vladimir },
	title     = {Non-contact stress measurement in granular
	materials via neutron and x-ray diffraction: theoretical foundations},
	journal = {Granular Matter},
	year      = {2013},
	volume    = {15},
	pages     = {275--286},
}

@article{chrisgranular,
	author    = {CM Wensrich and JN Hendriks, and MH Meylan },
	title     = {Bragg edge neutron transmission strain tomography in granular systems},
	journal = {Strain},
	year      = {2016},
	volume    = {52},
	pages     = {80--87},
}

@article{PhysRevApplied.10.064034,
	title = {Tomographic Reconstruction of Two-Dimensional Residual Strain Fields from Bragg-Edge Neutron Imaging},
	author = {Gregg, A.W.T. and Hendriks, J.N. and Wensrich, C.M. and Wills, A. and Tremsin, A.S. and Luzin, V. and Shinohara, T. and Kirstein, O. and Meylan, M.H. and Kisi, E.H.},
	journal = {Phys. Rev. Applied},
	volume = {10},
	issue = {6},
	pages = {064034},
	numpages = {11},
	year = {2018},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevApplied.10.064034},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.10.064034}
}

@article{Chris2016,
	title = {Bragg-edge neutron transmission strain tomography for in situ loadings},
	author = {C.M. Wensrich and J.N. Hendriks and A. Gregg and M.H. Meylan and V. Luzin and A.S. Tremsin},
	journal = {Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
	volume = {383},
	issue = {},
	pages = {52--58},
	year = {2016},
}

@article{braggedge1,
	title = {Strain Imaging by Bragg edge
	neutron transmission},
	author = {J.R. Santisteban and L. Edwards and M.E. Fitzpatrick and A. Steuwer and
	P.J. Withers and M.R. Daymond and M.W. Johnson and N. Rhodes,
	and EM Schooneveld},
	journal = {Nuclear Instruments and Methods
	in Physics Research Section A: Accelerators, Spectrometers,
	Detectors and Associated Equipment},
	volume = {481},
	issue = {},
	pages = {765--768},
	year = {2002},
}

@book{Beamprob,
	author  = {F. Beer and E.R. Jr. Johnston and J. DeWolf, and D. Mazurek },
	title   = {Mechanics of Materials},
	journal = {McGraw-Hill},
	year    = {2008},
	pages   = {},
	issn    = {},
}

@article{tof,
	author    = {AS Tremsin and JB McPhate and A Steuwer and W Kockelmann and
	A M Paradowska and JF Kelleher and JV Vallerga and OHW Siegmund and
	and WB Feller},
	title     = {High-resolution strain mapping
	through time-of-flight neutron transmission diffraction
	with a microchannel plate neutron counting detector},
	journal = {Strain},
	year      = {2012},
	volume    = {48},
	pages     = {296--305},
}

@article{detector,
	author    = {AS Tremsin and JB McPhate and W Kockelmann and JV Vallerga and
	OHW Siegmund, and WB Feller},
	title     = {High resolution
	Bragg edge transmission spectroscopy at pulsed
	neutron sources: proof of principle experiments with a
	neutron counting MCP detector},
	journal = {Nuclear Instruments
	and Methods in Physics Research Section A: Accelerators,
	Spectrometers, Detectors and Associated Equipment},
	year      = {2011},
	volume    = {633},
	pages     = {235--238},
}

@article{braggedge2,
	author    = {JR Santisteban and L Edwards and ME Fizpatrick and A Steuwer,
	and PJ Withers},
	title     = {Engineering applications of Bragg-edge
	neutron transmission},
	journal = {Applied Physics A},
	year      = {74},
	volume    = {2002},
	pages     = {1433--1436},
}


@article{lsqr,
	author    = {Christopher C Paige and Michael A Saunders},
	title     = { Lsqr: An algorithm for sparse linear
	equations and sparse least squares},
	booktitle = {},
	year      = {1982},
	volume    = {},
	pages     = {},
}
@book{kisi2012applications,
	title={Applications of neutron powder diffraction},
	author={Kisi, Erich H and Howard, Christopher J},
	volume={15},
	year={2012},
	publisher={Oxford University Press}
}

@book{fitzpatrick2003analysis,
	title={Analysis of residual stress by diffraction using neutron and synchrotron radiation},
	author={Fitzpatrick, Michael E and Lodini, Alain},
	year={2003},
	publisher={CRC Press}
}

@article{raden,
	title = {Final design of the Energy-Resolved Neutron Imaging System {"}rADEN{"} at J-PARC},
	author = {T. Shinohara and T. Kai and K. Oikawa and M. Segawa and M. Harada and T. Nakatani and M. Ooi and K. Aizawa and H. Sato and T. Kamiyama and H. Yokota and Toshihiro Sera and K. Mochiki and Y. Kiyanagi},
	year = {2016},
	volume = {746},
	journal = {Journal of Physics: Conference Series},
}

@article{wahba1990spline,
  title={Spline Models for Observational Data (Philadelphia, PA: Society for Industrial and Applied Mathematics)},
  author={Wahba, G},
  journal={Mathematical Reviews (MathSciNet): MR1045442 Zentralblatt MATH},
  volume={813},
  year={1990}
}

@article{jparc,
	author    = {Takenao Shinohara and Tetsuya Kai},
	title     = {Commissioning start of Energy-Resolved Neutron Imaging System, RADEN in J-PARC},
	journal   = {Neutron News},
	year      = {2015},
	volume    = {26},
	number    = {2},
	pages     = {11-14},


%@Comment{jabref-meta: databaseType:bibtex;}


==> bib.tex <==
% Encoding: UTF-8
@article{review,
  author={R. Woracek and Javier Santisteban and Anna Fedrigo and Markus Strobl},
  title={Diffraction in neutron imaging —- A review},
  year={2018},
  journal={Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
  volume={878},
  pages={141--158},
  publisher={}}

@article{golub1999tikhonov,
  title={Tikhonov regularization and total least squares},
  author={Golub, Gene H and Hansen, Per Christian and O'Leary, Dianne P},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={21},
  number={1},
  pages={185--194},
  year={1999},
  publisher={SIAM}
}
@article{inverse_prob,
  author    = {W. R. B. Lionheart and P. J. Withers},
  title     = {Diffraction tomography of strain},
  booktitle = {Inverse Problems},
  year      = {2015},
  volume    = {31},
  pages     = {045005},
}

@article{Kirkwood2015,
author ={Henry J. Kirkwood and Shu Yan Zhang and Anton S. Tremsin and Alexander M. Korsunsky and Nikolaos Baimpas and Brian Abbey},
title={Neutron Strain Tomography using the Radon Transform},
journal={Materials Today: Proceedings},
year={2015},
volume  = {2},
pages   = {S414--S423},
issn    = {},
}


@inproceedings{Gregg2017TomographicRO,
	title={Tomographic reconstruction of residual strain in axisymmetric systems from Bragg-edge neutron imaging},
	author={Alexander Gregg and Johannes N. Hendriks and Christopher Wensrich and Michael H. Meylan},
	year={2017}
}


@article{Abbey,
  author  = {B. Abbey and Shu Yan Zhang and Wim.J.J. Vorster and Alexander M. Korsunsky},
  title   = {Feasibility study of neutron strain tomography},
  journal = {Procedia Engineering},
  year    = {2009},
  volume  = {1},
  pages   = {185--188},
  issn    = {},
}
@article{Abbey12,
	author  = {B. Abbey and Shu Yan Zhang and Wim.J.J. Vorster and Alexander M. Korsunsky},
	title   = {Reconstruction of axisymmetric strain distributions via neutron strain tomography},
	journal = {Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
	year    = {2012},
	volume  = {270},
	pages   = {28--35},
	issn    = {},
}
@inproceedings{Sharafutdinov1994INTEGRALGO,
	title={INTEGRAL GEOMETRY OF TENSOR FIELDS},
	author={Vladimir A. Sharafutdinov},
	year={1994}
}



@article{Bragg_edge,
  author  = {Hendriks, J. N. and Gregg, A. W. T. and Wensrich, C. M. and Tremsin, A. S. and Shinohara, T. and Meylan, M. and Kisi, E. H. and Luzin, V. and Kirsten, O.},
  title   = {Bragg-edge elastic strain tomography for in situ systems from energy-resolved neutron transmission imaging},
  journal = {Phys. Rev. Materials},
  year    = {2017},
  volume  = {1},
  pages   = {053802},
  issn    = {},
}


@book{Gaussian,
  author  = {C. E. Rasmussen and C. K. I. Williams},
  title   = {Gaussian Processes for Machine Learning},
  journal = {MIT Press},
  year    = {2006},
  pages   = {},
  issn    = {},
  }

@article{Gauss_prob,
  author  = {C. Jidling and Johannes Hendriks and Niklas Wahlström and Alexander Gregg and Thomas B. Schön and Christopher Wensrich and Adrian Wills},
  title   = {Probabilistic modelling and reconstruction of strain},
  journal = {Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
  year    = {2018},
  pages   = {141--155},
  issn    = {},
  }


@article{AIP,
  author    = {C. M. Wensrich and Kisi, Erich and Luzin, Vladimir and Kirstein, Oliver},
  title     = {Non-contact Measurement of the Stress within Granular Materials via Neutron Diffraction},
  journal = {AIP Conference Proceedings},
  year      = {2013},
  volume    = {1542},
  pages     = {441--444},
}
@article{granular,
	author    = {C. M. Wensrich and Kisi, Erich and Luzin, Vladimir },
	title     = {Non-contact stress measurement in granular
	materials via neutron and x-ray diffraction: theoretical foundations},
	journal = {Granular Matter},
	year      = {2013},
	volume    = {15},
	pages     = {275--286},
}

@article{chrisgranular,
	author    = {CM Wensrich and JN Hendriks, and MH Meylan },
	title     = {Bragg edge neutron transmission strain tomography in granular systems},
	journal = {Strain},
	year      = {2016},
	volume    = {52},
	pages     = {80--87},
}

@article{PhysRevApplied.10.064034,
	title = {Tomographic Reconstruction of Two-Dimensional Residual Strain Fields from Bragg-Edge Neutron Imaging},
	author = {Gregg, A.W.T. and Hendriks, J.N. and Wensrich, C.M. and Wills, A. and Tremsin, A.S. and Luzin, V. and Shinohara, T. and Kirstein, O. and Meylan, M.H. and Kisi, E.H.},
	journal = {Phys. Rev. Applied},
	volume = {10},
	issue = {6},
	pages = {064034},
	numpages = {11},
	year = {2018},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevApplied.10.064034},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.10.064034}
}

@article{Chris2016,
	title = {Bragg-edge neutron transmission strain tomography for in situ loadings},
	author = {C.M. Wensrich and J.N. Hendriks and A. Gregg and M.H. Meylan and V. Luzin and A.S. Tremsin},
	journal = {Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
	volume = {383},
	issue = {},
	pages = {52--58},
	year = {2016},
}

@article{braggedge1,
	title = {Strain Imaging by Bragg edge
	neutron transmission},
	author = {J.R. Santisteban and L. Edwards and M.E. Fitzpatrick and A. Steuwer and
	P.J. Withers and M.R. Daymond and M.W. Johnson and N. Rhodes,
	and EM Schooneveld},
	journal = {Nuclear Instruments and Methods
	in Physics Research Section A: Accelerators, Spectrometers,
	Detectors and Associated Equipment},
	volume = {481},
	issue = {},
	pages = {765--768},
	year = {2002},
}

@book{Beamprob,
	author  = {F. Beer and E.R. Jr. Johnston and J. DeWolf, and D. Mazurek },
	title   = {Mechanics of Materials},
	journal = {McGraw-Hill},
	year    = {2008},
	pages   = {},
	issn    = {},
}

@article{tof,
	author    = {AS Tremsin and JB McPhate and A Steuwer and W Kockelmann and
	A M Paradowska and JF Kelleher and JV Vallerga and OHW Siegmund and
	and WB Feller},
	title     = {High-resolution strain mapping
	through time-of-flight neutron transmission diffraction
	with a microchannel plate neutron counting detector},
	journal = {Strain},
	year      = {2012},
	volume    = {48},
	pages     = {296--305},
}

@article{detector,
	author    = {AS Tremsin and JB McPhate and W Kockelmann and JV Vallerga and
	OHW Siegmund, and WB Feller},
	title     = {High resolution
	Bragg edge transmission spectroscopy at pulsed
	neutron sources: proof of principle experiments with a
	neutron counting MCP detector},
	journal = {Nuclear Instruments
	and Methods in Physics Research Section A: Accelerators,
	Spectrometers, Detectors and Associated Equipment},
	year      = {2011},
	volume    = {633},
	pages     = {235--238},
}

@article{braggedge2,
	author    = {JR Santisteban and L Edwards and ME Fizpatrick and A Steuwer,
	and PJ Withers},
	title     = {Engineering applications of Bragg-edge
	neutron transmission},
	journal = {Applied Physics A},
	year      = {74},
	volume    = {2002},
	pages     = {1433--1436},
}


@article{lsqr,
	author    = {Christopher C Paige and Michael A Saunders},
	title     = { Lsqr: An algorithm for sparse linear
	equations and sparse least squares},
	booktitle = {},
	year      = {1982},
	volume    = {},
	pages     = {},
}
@book{kisi2012applications,
	title={Applications of neutron powder diffraction},
	author={Kisi, Erich H and Howard, Christopher J},
	volume={15},
	year={2012},
	publisher={Oxford University Press}
}

@book{fitzpatrick2003analysis,
	title={Analysis of residual stress by diffraction using neutron and synchrotron radiation},
	author={Fitzpatrick, Michael E and Lodini, Alain},
	year={2003},
	publisher={CRC Press}
}

@article{raden,
	title = {Final design of the Energy-Resolved Neutron Imaging System {"}rADEN{"} at J-PARC},
	author = {T. Shinohara and T. Kai and K. Oikawa and M. Segawa and M. Harada and T. Nakatani and M. Ooi and K. Aizawa and H. Sato and T. Kamiyama and H. Yokota and Toshihiro Sera and K. Mochiki and Y. Kiyanagi},
	year = {2016},
	volume = {746},
	journal = {Journal of Physics: Conference Series},
}

@article{wahba1990spline,
  title={Spline Models for Observational Data (Philadelphia, PA: Society for Industrial and Applied Mathematics)},
  author={Wahba, G},
  journal={Mathematical Reviews (MathSciNet): MR1045442 Zentralblatt MATH},
  volume={813},
  year={1990}
}

@article{jparc,
	author    = {Takenao Shinohara and Tetsuya Kai},
	title     = {Commissioning start of Energy-Resolved Neutron Imaging System, RADEN in J-PARC},
	journal   = {Neutron News},
	year      = {2015},
	volume    = {26},
	number    = {2},
	pages     = {11-14},


%@Comment{jabref-meta: databaseType:bibtex;}

